PILOT: Password and PIN Information Leakage from Obfuscated Typing Videos

This paper studies leakage of user passwords and PINs based on observations of typing feedback on screens or from projectors in the form of masked characters that indicate keystrokes. To this end, we developed an attack called Password and Pin Information Leakage from Obfuscated Typing Videos (PILOT). Our attack extracts inter-keystroke timing information from videos of password masking characters displayed when users type their password on a computer, or their PIN at an ATM. We conducted several experiments in various attack scenarios. Results indicate that, while in some cases leakage is minor, it is quite substantial in others. By leveraging inter-keystroke timings, PILOT recovers 8-character alphanumeric passwords in as little as 19 attempts. When guessing PINs, PILOT significantly improved on both random guessing and the attack strategy adopted in our prior work [4]. In particular, we were able to guess about 3% of the PINs within 10 attempts. This corresponds to a 26-fold improvement compared to random guessing. Our results strongly indicate that secure password masking GUIs must consider the information leakage identified in this paper.

==> gfx/passwords/combined_plain/results <==
ALL
123brian
183
jillie02
186
william1
183
lamondre
184
RF
\texttt{123brian} & 581743 & 414761 & 508332 & 57.92\% & 93874 & 8.74\% & 5535 & 1.09\% & 3.28\% & 9.29\%\\
\texttt{jillie02} & 749718 & 448319 & 656754 & 56.45\% & 1753571 & 97.85\% & 28962 & 0.00\% & 0.54\% & 2.69\%\\
\texttt{william1} & 246437 & 264090 & 145966 & 64.48\% & 187 & 0.55\% & 68 & 10.93\% & 23.50\% & 39.89\%\\
\texttt{lamondre} & 301906 & 334681 & 199344 & 66.85\% & 397213 & 75.00\% & 145 & 13.04\% & 19.57\% & 33.70\%\\
NN
\texttt{123brian} & 923534 & 165454 & 886802 & 58.47\% & 93874 & 0.00\% & 577739 & 0.00\% & 0.00\% & 0.00\%\\
\texttt{jillie02} & 456811 & 210512 & 383230 & 63.44\% & 1753571 & 100.00\% & 164754 & 0.00\% & 0.00\% & 0.00\%\\
\texttt{william1} & 265813 & 140753 & 215840 & 63.39\% & 187 & 0.00\% & 45176 & 0.00\% & 0.55\% & 3.83\%\\
\texttt{lamondre} & 517472 & 189355 & 493713 & 57.07\% & 397213 & 28.80\% & 148403 & 0.00\% & 0.00\% & 0.00\%\\

